OCEAN: Open-source Collation of eGovernment data And Networks - Understanding Privacy Leaks in Open Government Data

The awareness and sense of privacy has increased in the minds of people over the past few years. Earlier, people were not very restrictive in sharing their personal information, but now they are more cautious in sharing it with strangers, either in person or online. With such privacy expectations and attitude of people, it is difficult to embrace the fact that a lot of information is publicly available on the web. Information portals in the form of the e-governance websites run by Delhi Government in India provide access to such PII without any anonymization. Several databases e.g., Voterrolls, Driving Licence number, MTNL phone directory, PAN card serve as repositories of personal information of Delhi residents. This large amount of available personal information can be exploited due to the absence of proper written law on privacy in India. PII can also be collected from various social networking sites like Facebook, Twitter, GooglePlus etc. where the users share some information about them. Since users themselves put this information, it may not be considered as a privacy breach, but if the information is aggregated, it may give out much more information resulting in a bigger threat. To bring such issues to public notice, we developed Open-source Collation of eGovernment data And Networks (OCEAN), a system where the user enters little information (e.g. Name) about a person and gets large amount of personal information about him / her like name, age, address, date of birth, mother's name, father's name, voter ID, driving licence number, PAN.

==> mtech.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\@setckpt{mtech\unhbox \voidb@x \penalty \@M \hskip \z@skip \unhbox \voidb@x \kern .06em\vbox {\hrule width.3em}\discretionary {-}{}{}\penalty \@M \hskip \z@skip thesis\unhbox \voidb@x \penalty \@M \hskip \z@skip \unhbox \voidb@x \kern .06em\vbox {\hrule width.3em}\discretionary {-}{}{}\penalty \@M \hskip \z@skip cover}{
\setcounter{page}{2}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{chapter}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{ContinuedFloat}{0}
\setcounter{AlgoLine}{0}
\setcounter{algocfline}{0}
\setcounter{algocfproc}{0}
\setcounter{algocf}{0}
\setcounter{Item}{0}
\setcounter{Hfootnote}{0}
\setcounter{bookmark@seq@number}{0}
\setcounter{r@tfl@t}{0}
\setcounter{parentequation}{0}
\setcounter{float@type}{4}
\setcounter{section@level}{0}
}

